Querying in the Age of Graph Databases and Knowledge Graphs

Graphs have become the best way we know of representing knowledge. The computing community has investigated and developed the support for managing graphs by means of digital technology. Graph databases and knowledge graphs surface as the most successful solutions to this program. The goal of this document is to provide a conceptual map of the data management tasks underlying these developments, paying particular attention to data models and query languages for graphs.

==> about.tex <==

\claudio{esta seccion esta lista para ser eliminada. 
Lleve un parrafo a la intro,
y otro a la seccion 2. Estos dos
que quedan se pueden
pasar ahora a la seccion siguiente
donde sean necesarias estas defns.}


%Traditional database problems can be found in graph databases and knowledge graphs. In particular, the problems of constructing a database in the appropriate data model, integrating sources with different formats and even with contradicting semantics, developing methods to extract information, encapsulating such methods in query languages, incorporating reasoning capabilities to deduce new knowledge, developing analytic techniques to improve our understanding of the structure and content of a database as a whole, and providing visualization techniques for exploring and querying the data. But we see a new trend in knowledge graphs, where the continuous interaction between representation, integration and production of knowledge has made inductive methods play a crucial role. Two important examples of this are knowledge graph embeddings \cite{CZC18} and graph neural networks \cite{ML05,SGTHM09}.



On one side, a knowledge graph embedding is a map that  represents a graph in a low-dimensional vector space. For example, assuming that $\cL = (N,E,\rho,\lambda)$ is a labeled graph, an embedding can be a function $f : (N \cup E) \to \mathbb{R}^d$, where $d \geq 1$. Such a function should reflect the structure of the graph as accurately as possible: an edge in the graph should become a geometric relation in the vector space, while such a geometric relation should not hold for an edge not occurring  in the graph. Notice that under an open-world assumption, one may need to explicitly specify the edges that do not occur in the graph. For example, if $\rho(e) = (n_1,n_2)$, we expect that $f(n_1) + f(e) = f(n_2)$. In a broader sense, these geometric relations can be approximated, for example measuring how close $\|f(n_1) + f(e) - f(n_2)\|$ is to $0$ \cite{BUGWY13}, o they can be replaced by more general plausibility functions \cite{CZC18}. In line with what is mentioned in the previous paragraph, embeddings have played a crucial role in knowledge graph construction, refinement and completion \cite{LLSLZ15,P17}. In fact, they have even been used to answer more complex logical queries, which might need to deal with multiple unobserved nodes and edges in a graph \cite{HBZJL18,RHL20}.
 
On the other side, a graph neural network is a neural network that receives as input a graph, and produces a graph where each node is associated with a vector of features. Besides, it has a classification function that returns a Boolean value either \textit{true} or \textit{false} for each node. In this way, a graph neural network is a classifier~\cite{ML05,SGTHM09}, but it can also be viewed as a query \cite{BKMPRS20} that holds for the nodes that are classified as true. Again, in line with what is mentioned before, graph neural networks are widely used to extract knowledge from graphs. 
 
%The goal of the rest of this tutorial is to provide a unified and simple view of the data models behind graph databases and knowledge graphs, and then show some recently established results on querying such graphs. More specifically, we focus on the fundamental task of extracting knowledge from graphs in the form of nodes and paths satisfying a pattern, and we study new paradigms on path extraction, the inclusion of knowledge in some graph analytic tasks, and the connection of declarative with procedural frameworks for node extraction.


==> history.tex <==

\marcelo{Voy a ir agregando aquí citaciones que me parecen relavantes.}

\cite{AABHRV17,DBLP:journals/corr/abs-2003-02320,GS21,FSAHKPTUW20}



==> why_tutorial.tex <==


When addressing graphs as a model for data to knowledge, we cannot ignore the obvious: the knowledge graph hype. 
Knowledge Graphs can be seen as fulfilling an early vision in Computer Science of creating intelligent systems that integrate and manage knowledge and data at large scale. 
Computer Science publications about knowledge graphs stems from areas such as semantic web, databases, various sub areas of AI including knowledge representation and reasoning, natural language processing, machine learning among many others. 
There is not a single agreed upon definition for knowledge graph. 
As noted in 
%As Hogan et al notes
\cite{DBLP:journals/corr/abs-2003-02320}, ``{\em definition of a `knowledge graph' remains contentious, where a number of (sometimes conflicting) definitions have emerged, varying from specific technical proposals to more inclusive general proposals}"\footnote{We refer the reader to Appendix A of \cite{DBLP:journals/corr/abs-2003-02320} for the various definitions of Knowledge Graphs.}, however they provide an inclusive definition for a knowledge graph: 
{\em "a graph of data intended to accumulate and convey knowledge of the real world, whose nodes represent entities of interest and whose edges represent relations between these entities."}

Given the hype, it is important to ask ourselves what is new with knowledge graphs? 
Let us start by observing what is known about knowledge graphs. 
The popularity of the term "knowledge graph" stems from Google's Knowledge Graph announcement in 2012.\footnote{https://blog.google/products/search/introducing-knowledge-graph-things-not/}
Nevertheless, there is a rich history of scientific contributions leading to emergence of knowledge graphs. 
In \cite{GS21}, the authors 
%Gutierrez and Sequeda 
provide historical context for the roots of knowledge graphs grounded in the advancements of the computer science disciplines of knowledge, data, and the combination thereof. %\cite{GS21}.
Throughout the past 50 years, the knowledge and data disciplines have provide independent advances, 
%but 
%there have always been attempts to combine knowledge and data together.
and 
there have been multiple attempts to combine them. 
Knowledge graphs is a modern manifestation of the phenomena of combining knowledge and data.
%On the knowledge side: semantic networks, knowledge representation and reasoning languages, 
%On the data side: relational model, database management systems, graph theory.
%Furthermore, knowledge and data has been interweaving and providing results such as deductive databases, semantic web, 

The knowledge graph hype can be informed by the quantity of publications throughout this past decade. Let’s first start by analyzing knowledge graph related papers which we define as pub- lications that have the strings "knowledge graph", "RDF", "SPARQL"
"graph database" and "property graph" in their title.\footnote{
3We acknowledge that this is not a thorough analysis, nevertheless, it should be sufficient to shed light to the knowledge graph hype phenomena.
}
Between 2010
and 2020, there has been a total of 6139 knowledge graph publications that appear indexed by DBLP.\footnote{
This includes all types of publications indexed by DBLP: journal, conferences, work- shops, editorship, etc.
}
Figure 1 shows the number of
publications of the knowledge graph related papers from 2010 to 2020.

\begin{figure}[h]
\includegraphics[width=9cm]{knowledge-graph1.png}
\caption{Number of knowledge graph related publications. Source: DBLP.}
\label{fig:KGDBLP}
\end{figure}

We observe the following.
The growth of "knowledge graph" papers can be seen starting in 2013, which correlates with the year after the Google's Knowledge Graph announcement. 
The amount of publications about "RDF" and "SPARQL" continue to be stable. However we observe a decline when compared to "knowledge graph". 
In 2015, 70\% of knowledge graphs papers were about RDF/SPARQL, while that went down to 14\% in 2020.
Papers about "graph database" are very small and there is no significant growth, while papers about "property graph" are negligible.
The main takeaway message from this is that publications about knowledge graphs are significantly increasing, and in the past years with the usage of the term "knowledge graph". 

A follow up questions is: where are these papers being published? 
Figure~\ref{fig:KG-Venues-DBLP} provides an answer to this question.
Semantic Web venues have the strings Semantic Web, ISWC, ESWC, WWW and J. Web Semant in the title of the venue.
Database venues have the strings SIGMOD, VLDB, EDBT, ICDT, PODS, ICDE, Trans. Know, Trans. Database in the title of the venue. 
AI/ML/NLP venues have the strings AAAI, IJCAI, Neuro, NeurIPS, ICLR, EMNLP, ACL, COLING in the title of the venue.

\begin{figure}[h]
\includegraphics[width=9cm]{knowledge-graph2.png}
\caption{Number of knowledge graph related papers published in Semantic Web, AI/ML/NLP, Database and arXiv venues. Source: DBLP.}
\label{fig:KG-Venues-DBLP}
\end{figure}

We observe the following about knowledge graph related publications:
they have been low and stable at database venues;
they are higher in semantic web venues;
they have been low and stable at AI/ML/NLP venues, until 2019 where they have increased 3X; 
and they have been increasing at arXiv, where a jump is observed in 2018 when it overcomes semantic web venues. 
Besides, on average, 40\% of knowledge graph related articles are published in arXiv and Semantic Web, Database, and AI/ML/NLP venues combined. 
The rest of the publications observed at DBLP are distributed in a very long tail.


The main takeaway message here is that the database community does not seem to be on-board the knowledge graph hype. 
Given this, we ask ourselves whether the database community should care about this hype.
How much of the research under the name of "knowledge graphs" is new? 
How much is this different from what is already known in the  database community? 

The goal of this tutorial is to reflect and spark the discussion on these questions.
Is this a hype that the database community should be paying attention to, because there are new problems and we have a lot to contribute? 
Or is this a hype with a lot of noise, and it will pass? 
In other words, should the database community be riding the knowledge graph wave or is it safe to ignore? 
We believe that we cannot talk about graph databases without talking about knowledge graph. 

\marcelo{Aquí tenemos que poner un párrafo diciendo sobre lo que vamos a ver en las siguientes secciones.}


% Graph are a natural way to represent information (Claudio)


% There is a lot of hype around knowledge graphs.
% \begin{itemize}
%     \item What are knowledge graphs? Is there anything new? (Claudio)
    
%     \item Why are knowledge graph so popular? See the trend in publications.
    
%     \item We offer an analysis of the trend of publications, with an emphasis on databases and artificial intelligence (Juan/Marcelo). 
% \end{itemize}
% Based on the previous analysis, we identify the following research problems that are being studied today:
%   \claudio{seria interesante agrupar esta lista de supermercado en temas mas 
%   conceptuales. Imagino: representation of KG (embeddings; text; images);  
%   enhancement of knowledge (completion,  ); integrating knowledge ( ....);
%   obtaining/producing knowledge (learning, mining, etc.), etc.}
% \begin{itemize}
%     \item Knowledge graph embeddings \cite{CZC18}. 
    
%     \item Knowledge graph completion/link prediction/refinement: to predict unobserved or missing edges between entities \cite{LLSLZ15}.
%     \marcelo{Está parece ser un área gigante, estoy empezando a ver la literatura sobre esto.}
    
%     \item About the previous topic, techniques to  handle more complex logical queries (like conjunctive queries) have been proposed, which might need to deal with multiple unobserved edges and entities in a graph \cite{HBZJL18,RHL20}.
%     \marcelo{Me parece interesante mencionar esto porque desafia el limite entre bases de datos y machine learning, al tratar de usar técnicas de machine learning para aprender algoritmos para evaluar conjunctive queries. ¿Tiene sentido hacer esto? En particular considerando que los algoritmos generados van a ser aproximados}
%     \marcelo{En el estudio sobre las publicaciones deberíamos ver si este es un tópico popular.}
    
    
%     \item Alignment/Integration 
    
%     \item Knowledge graph generation/construction
    
%     \item Knowledge graph manipulation
    
%     \item Visualization: as a form of querying? Visual query languages.
    
%     \item Keyword queries
    
%     \item: Reasoning: are reasoning capabilities really needed? How much is really needed?
    
%     \item Query answering
    
%     \item Modelling applications.
    
%     \item Exploring and Querying Knowledge Graphs.
% \end{itemize}


% ¿Qué va a aprender en este tutorial?

% ¿Qué se entiende por un KG? ¿Hay algo nuevo? (Secciones 2 y 3)

% Modelos: cuatro grandes paradigmas


% \marcelo{Preguntas recopiladas por Juan desde EDBT/ICDT}

% Questions we should answer in this tutorial

% - "Whatever is being done with knowledge  seems to be done with data (integration, querying, relational/non-relational backends). Are there questions that distinguish research on knowledge from research on data?" Sihem Amer-Yahia

% - "After more than 20 years of research on semantic nets/graphs I am wondering what are the issues that still remain open" Vassilis Christophides

% - "How do you think we can build a bridge to the statistical community, which is inteterestd in modeling uncertainty and forms of connected knowledge? We have seen there is weak connection with the machine learning community, for instance" Eleonara Laurenza

% - What is the typical scale fo datasets and experiments? thousanda of nodes, millions of nodes, more? - Felix Naumann



